Collaborative Speculative Inference for Efficient LLM Inference Serving

Speculative inference is a promising paradigm employing small speculative models (SSMs) as drafters to generate draft tokens, which are subsequently verified in parallel by the target large language model (LLM). This approach enhances the efficiency of inference serving by reducing LLM inference latency and costs while preserving generation quality. However, existing speculative methods face critical challenges, including inefficient resource utilization and limited draft acceptance, which constrain their scalability and overall effectiveness. To overcome these obstacles, we present CoSine, a novel speculative inference system that decouples sequential speculative decoding from parallel verification, enabling efficient collaboration among multiple nodes. Specifically, CoSine routes inference requests to specialized drafters based on their expertise and incorporates a confidence-based token fusion mechanism to synthesize outputs from cooperating drafters, ensuring high-quality draft generation. Additionally, CoSine dynamically orchestrates the execution of speculative decoding and verification in a pipelined manner, employing batch scheduling to selectively group requests and adaptive speculation control to minimize idle periods. By optimizing parallel workflows through heterogeneous node collaboration, CoSine balances draft generation and verification throughput in real-time, thereby maximizing resource utilization. Experimental results demonstrate that CoSine achieves superior performance compared to state-of-the-art speculative approaches. Notably, with equivalent resource costs, CoSine achieves up to a 23.2% decrease in latency and a 32.5% increase in throughput compared to baseline methods.

==> chap2/relatedwk.tex <==
\section{Related Work}
% \textbf{Multi-Token Predictions. } 
% Since Stern \cite{}, predicting the next k tokens simultaneously has proven effective, but it requires adding k feed-forward decoder layers from the last encoder state. Cai popularized this idea using Medusa heads, additionally predicting multiple token branches using tree attention.
% In the SpecDec \cite{} method, multitoken prediction is done by unmasking future tokens from multiple decoder heads attending to different encoder states, utilizing distinct attention queries for predicting different tokens. However, SpecDec requires full model fine-tuning for all layers as the decoder-only target model has not been pretrained on multi-token unmasking tasks. More recently, Bhendawade \cite{} predict multiple tokens by adding streaming embeddings initialized from upper layers, with the token tree reduced by early exiting. However, they made major changes to the original architecture, and their speedups are considered limited.
% Multi-token prediction can also be implemented auto-regressively \cite{}, which takes multiple steps to predict the next draft token conditioned on previously drafted tokens in one iteration. To mitigate the substantial overheads incurred by multistep drafting within a single iteration, the draft overhead should be minimal while ensuring it retains the capability to generate acceptable tokens. In the case of EAGLE \cite{li2024eagle}, this is achieved by efficiently concatenating the target model’s high-level features with the embeddings or hidden states of the next tokens for regression via an additional layer of Transformer decoder.
% Handling large memory footprint in LLM is challenging, as bothLLM parameters and KV cache are stored in memory. 
% Another line of work to generate multiple draft tokens in parallel is based on Jacobi iteration methods, treating auto-regressive decoding in LLM as a non-linear system of equations, or Jacobi decoding \cite{}. In practice, however, an LLM may obtain marginal speedups from Jacobi decoding as it can rarely produce an accepted token if a previous token in the trajectory is predicted incorrectly. Lookahead decoding \cite{} attempts to address this issue by introducing memory costs and caching n-gram tokens from previous Jacobi trajectories. Inspired by the Consistency Model \cite{}, CLLMs \cite{} additionally train their target models to minimize the distances between Jacobi trajectories and the fixed point, leading to faster convergence and thus greater speedups \cite{}. Compared to regular SD methods, Jacobi decoding does not have a separate draft phase.

% \textbf{Parallelism LLM Inference}
% Handling large memory footprint in LLM is challenging, as both
% LLM parameters and KV cache are stored in memory.  

\textbf{Speculative decoding} has previously been explored through Staged Speculative Decoding and SpecInfer \cite{miao2024specinfer}. %
SpecInfer utilized multiple speculative models executed in parallel with each other, but did not run the speculative and target models in parallel, resulting in increased end-to-end latency. 
Staged Speculative Decoding took a slightly different approach, where the speculative models were themselves speculatively inferenced, as the staged speculations were also not run in parallel with their respective targets. %
SpecInfer utilized multiple speculative models executed in parallel with each other, but did not run the speculative and target models in parallel, resulting in increased end-to-end latency. %

Medusa \cite{cai2024medusa} takes a slightly different approach to speculative decoding, adding new sampling heads to the target model that produce the speculations without a speculative model. Medusa does not incur significant latency overhead but requires training new sampling heads for the target model. %
Lookahead Decoding \cite{fu2024break} takes a different approach entirely, opting to use Jacobi iteration to generate multiple tokens simultaneously by generating N-grams based on the trajectory of the current tokens. 
Lookahead Decoding exhibits high utilization and low latency on single-node systems, but does not account for multi-node systems or systems with slow interconnects.%


